Controllable GAN Synthesis Using Non-Rigid Structure-from-Motion

In this paper, we present an approach for combining non-rigid structure-from-motion (NRSfM) with deep generative models,and propose an efficient framework for discovering trajectories in the latent space of 2D GANs corresponding to changes in 3D geometry. Our approach uses recent advances in NRSfM and enables editing of the camera and non-rigid shape information associated with the latent codes without needing to retrain the generator. This formulation provides an implicit dense 3D reconstruction as it enables the image synthesis of novel shapes from arbitrary view angles and non-rigid structure. The method is built upon a sparse backbone, where a neural regressor is first trained to regress parameters describing the cameras and sparse non-rigid structure directly from the latent codes. The latent trajectories associated with changes in the camera and structure parameters are then identified by estimating the local inverse of the regressor in the neighborhood of a given latent code. The experiments show that our approach provides a versatile, systematic way to model, analyze, and edit the geometry and non-rigid structures of faces.

==> sec/0-scratchpad.tex <==

\newpage
\appendix
\section{Old figures}

\subsection{method figure}

% Method intro figure
Figure~\ref{fig:method_old} illustrates of our proposed editing framework. Starting with a given latent code $\mathbf{w}$, the trained regressor $\phi$ predicts the rank-one parameters $\mathbf{q}$. 
These parameters can then be edited resulting in the perturbed parameters $\tilde{\mathbf{q}}$, which can be transformed to the edited latent code $\tilde{\mathbf{w}}$ by the transformation $\Omega$.
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/overview_v07.pdf}
    \caption{
    \red{[2DO] update this figure}    
    Illustration of the proposed editing framework. Starting from one latent code $\vec{w}$ we can generate an image $g(\mathbf{w}) = I$, and the corresponding rank-one model parameters $\vec{q}$, which describe a 2D face shape.
    To edit the original image, we edit the model parameters ${\vec{q}} \rightarrow \tilde{\vec{q}}$, transform them to the edited latent vector $\widetilde{\vec{w}}$, from which the edited image $g(\tilde{\mathbf{w}}) = \widetilde{I}$ is inferred by the generator $G$. 
%(1) input: images and landmarks => camera and 3D basis shapes, (2) MLP receives latent code gives  
    }
    \label{fig:method_old}
\end{figure}

\subsection{Basis shapes}
In Figure~\ref{fig:basisshapes_old} we show an illustration of the first 8 non-rigid basis shapes recovered with landmarks extracted from random samples of a StyleGAN2 \cite{Karras2020StyleGANada} generator trained on FFHQ. 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/fig-basisshapes.png}
    \caption{The first eight 3D non-rigid basis shapes.}
    \label{fig:basisshapes_old}
\end{figure}


\subsection{Editing framework}
Figure~\ref{fig:spaces_old} illustrates the editing framework. Starting with a given latent code $\mathbf{w}_0$, the trained regressor $\phi$ predicts the rank-one parameters $\mathbf{q}$. 
Edits on these parameters then yields the perturbed parameters $\tilde{\mathbf{q}}$, which can be used to transform $\mathbf{w}$ to the edited latent code $\tilde{\mathbf{w}}$ by the transformation $\Omega_{\mathbf{w}_0}$.
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/overview_spaces07.pdf}
    \caption{
        \red{[2DO] update this figure}   
        Illustration of the proposed editing framework. Starting from one latent code $\vec{w}$ we can generate an image $I$, and the corresponding rank-one model parameters $\vec{q}$, which describe a 2D face shape.
    To edit the original image, we edit the model parameters ${\vec{q}} \rightarrow \tilde{\vec{q}}$, transform them to the edited latent vector $\widetilde{\vec{w}}$, from which the edited image $\widetilde{I}$ is inferred by the generator $G$. 
    }
    \label{fig:spaces_old}
\end{figure}

\subsection{Snippet: orthogonality}
i.e. for $i,j>0$ we have 
\begin{align}
    \begin{split}
        \langle \mathbf{B}_i,\mathbf{B}_j \rangle 
        &= \langle \text{vec}(\mathbf{B}_i),\text{vec}(\mathbf{B}_j) \rangle\\
        &= \langle \mathbf{d}_i,\mathbf{d}_j \rangle
          \langle \mathbf{b}_i,\mathbf{b}_j \rangle = \delta_{ij}            
    \end{split}
\end{align}
%\red{How about $\langle (\mathbf{d}_i),(\mathbf{d}_j) \rangle$ ? they cannot be ortho*normal* }
where $\delta_{ij}$ is the dirac delta. 
Orthonormality follows directly from the fact that $\mathbf{b}_k$ is the $k$th right singular vectors of $\delta\matr{X}$ and that $\norm{\mathbf{d}_k} = 1$ for all $k$ by construction. 
